Lower-Resource, Higher Scores: Language Bias in LLM Evaluators

LLM evaluators (trained reward models and prompted LLM-as-a-Judge) are routinely validated via pairwise accuracy. In a multilingual setting, this operates under the premise that high pairwise accuracy implies reliable, language-neutral scoring. We show that this assumption does not hold. We conduct experiments with semantically identical instruction-response pairs across 23 languages, and find that multilingual evaluators assign significantly different scores to different evaluation languages. The bias is statistically significant and consistent across eight open-weight evaluators of different architectures and training paradigms, persists in frontier judges, and is strongly correlated with language resource level: lower-resource languages are scored more generously. Meanwhile, these biases are invisible to pairwise accuracy: evaluators achieve above 90% pairwise accuracy, yet have up to 43% difference in acceptance rate across languages under a global decision threshold, meaning, for instance, that harmful content in lower-resource languages is more likely to pass safety filters. Per-language thresholds would require language identification, which can be defeated by code-switched prompts. We then investigate why lower-resource languages receive higher rather than lower scores, and we find that model uncertainty is linked with the effect: models tend to give higher scores when less confident, both under negative log-likelihood and under token-free uncertainty measures; however, language identity remains a significant predictor after controlling for uncertainty, and the bias cannot be explained away by content difficulty alone, but is a structural, language-level misalignment.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> mechanistic_outputs/tab_mediation.tex <==
\begin{table}[t]
\centering
\small
\caption{Mediation analysis: language coefficients from standardized-score regressions, with and without NLL as a covariate. The ``Total'' column shows each language's coefficient relative to Arabic (reference) when only language dummies, model, and dataset indicators are included. The ``Direct'' column adds NLL and token count. The ``Mediated'' column shows the portion absorbed by NLL. Positive mediation percentages indicate that NLL partially explains why that language receives different scores.}
\label{tab:mediation}
\begin{tabular}{lcccc}
\toprule
\textbf{Lang} & \textbf{Total} & \textbf{Direct} & \textbf{Mediated} & \textbf{\% Mediated} \\
\midrule
  en & -0.3979 & -0.3855 & -0.0124 & 3.1\% \\
  zh & -0.3216 & -0.3095 & -0.0122 & 3.8\% \\
  id & -0.3033 & -0.3014 & -0.0019 & 0.6\% \\
  fr & -0.2413 & -0.2409 & -0.0003 & 0.1\% \\
  es & -0.2312 & -0.2271 & -0.0041 & 1.8\% \\
  pt & -0.2050 & -0.2013 & -0.0038 & 1.8\% \\
  ja & -0.1822 & -0.1791 & -0.0031 & 1.7\% \\
  de & -0.1740 & -0.1736 & -0.0004 & 0.2\% \\
  nl & -0.1323 & -0.1329 & 0.0006 & -0.5\% \\
  it & -0.1301 & -0.1294 & -0.0007 & 0.5\% \\
  ko & -0.0907 & -0.0896 & -0.0012 & 1.3\% \\
  ru & -0.0736 & -0.0734 & -0.0002 & 0.3\% \\
  vi & -0.0698 & -0.0668 & -0.0030 & 4.3\% \\
  pl & -0.0505 & -0.0564 & 0.0060 & -11.8\% \\
  tr & -0.0452 & -0.0436 & -0.0016 & 3.6\% \\
  cs & -0.0429 & -0.0462 & 0.0033 & -7.8\% \\
  fa & -0.0346 & -0.0389 & 0.0043 & -12.5\% \\
  ro & -0.0310 & -0.0374 & 0.0064 & -20.7\% \\
  hi & -0.0060 & -0.0398 & 0.0338 & -566.3\% \\
  uk & 0.0015 & -0.0063 & 0.0077 & 521.3\% \\
  he & 0.0024 & -0.0251 & 0.0275 & 1131.5\% \\
  el & 0.1390 & 0.1027 & 0.0363 & 26.1\% \\
\midrule
  \textit{Mean $|$coeff$|$} & 0.1321 & 0.1321 & — & -0.0\% \\
\bottomrule
\end{tabular}
\end{table}

==> mechanistic_outputs/tab_partial_regression.tex <==
\begin{table}[h]
\centering
\small

\begin{tabular}{lcccccc}
\toprule
 & \multicolumn{2}{c}{\textbf{NLL}} & \multicolumn{2}{c}{\textbf{Resource}} & \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
\textbf{Specification} & $\beta$ & $p$ & $\beta$ & $p$ & \textbf{Adj.\ $R^2$} \\
\midrule
\multicolumn{6}{l}{\textit{Language-level (N = 23)}} \\
  Score $\sim$ NLL & 0.000587 & 0.0000 & — & — & 0.532 \\
  Score $\sim$ Resource & — & — & -1.1232 & 0.0000 & 0.554 \\
  Score $\sim$ NLL + Resource & 0.000311 & 0.0731 & -0.6761 & 0.0407 & 0.603 \\
\midrule
\multicolumn{6}{l}{\textit{Item-level (N = 36,800)}} \\
  Score $\sim$ NLL + Tokens + C(lang) + C(model) + C(dataset) & -9.24e-05$^{***}$ & 0.0000 & — & — & 0.784 \\
  Score $\sim$ NLL + Tokens + Resource + C(model) + C(dataset) & -8.79e-05$^{***}$ & 0.0000 & -1.061$^{***}$ & 0.0000 & 0.783 \\
  Score $\sim$ NLL + Tokens + Resource + C(lang) + C(model) + C(dataset) & -9.24e-05$^{***}$ & 0.0000 & -0.755$^{***}$ & 0.0000 & 0.784 \\
\bottomrule
\end{tabular}
\caption{Partial regression analysis disentangling NLL and resource level effects on reward scores. \textit{Top:} Language-level regressions (23 languages, scores averaged across models). \textit{Bottom:} Item-level regressions (36,800 items). NLL retains significant predictive power even after controlling for resource availability. Replacing language fixed effects with a continuous resource measure causes only a modest drop in $R^2$, suggesting NLL partially mediates the language effect. Significance: $^{***}p<0.001$, $^{**}p<0.01$, $^{*}p<0.05$.}
\label{tab:partial_regression}
\end{table}

==> mechanistic_outputs/tab_within_language.tex <==
\begin{table}[h]
\centering
\small

\begin{tabular}{lccccc}
\toprule
\textbf{Lang} & \textbf{Mean $\beta_\text{NLL}$} & \textbf{Median $\beta_\text{NLL}$} & \textbf{\% Positive} & \textbf{Sig.\ (p<.05)} & \textbf{Mean $R^2$} \\
\midrule
  ko & 0.00055 & 0.00014 & 75\% & 2/4 & 0.0250 \\
  hi & 0.00030 & 0.00010 & 75\% & 2/4 & 0.0244 \\
  cs & 0.00028 & 0.00006 & 75\% & 3/4 & 0.0190 \\
  ar & 0.00028 & 0.00010 & 75\% & 1/4 & 0.0170 \\
  pl & 0.00027 & 0.00010 & 75\% & 2/4 & 0.0324 \\
  nl & 0.00026 & 0.00005 & 75\% & 2/4 & 0.0158 \\
  el & 0.00024 & 0.00013 & 75\% & 2/4 & 0.0388 \\
  en & 0.00023 & -0.00002 & 50\% & 2/4 & 0.0106 \\
  fr & 0.00023 & 0.00006 & 75\% & 1/4 & 0.0088 \\
  he & 0.00023 & 0.00014 & 75\% & 3/4 & 0.0226 \\
  it & 0.00021 & 0.00012 & 75\% & 2/4 & 0.0160 \\
  tr & 0.00019 & 0.00008 & 75\% & 1/4 & 0.0172 \\
  ro & 0.00019 & 0.00009 & 75\% & 1/4 & 0.0112 \\
  zh & 0.00017 & -0.00000 & 50\% & 1/4 & 0.0068 \\
  ru & 0.00016 & 0.00009 & 75\% & 2/4 & 0.0178 \\
  pt & 0.00013 & 0.00008 & 75\% & 1/4 & 0.0101 \\
  de & 0.00013 & 0.00009 & 75\% & 1/4 & 0.0090 \\
  fa & 0.00013 & 0.00006 & 100\% & 1/4 & 0.0173 \\
  ja & 0.00011 & 0.00008 & 75\% & 2/4 & 0.0107 \\
  vi & 0.00010 & 0.00005 & 50\% & 1/4 & 0.0097 \\
  es & 0.00010 & 0.00006 & 75\% & 2/4 & 0.0151 \\
  uk & 0.00006 & 0.00008 & 75\% & 2/4 & 0.0197 \\
  id & -0.00005 & 0.00002 & 75\% & 2/4 & 0.0230 \\
\midrule
\textit{Overall} & 0.00020 & 0.00009 & 73\% & 39/92 & 0.0173 \\
\bottomrule
\end{tabular}
\caption{Within-language instance-level regressions: Score $\sim$ NLL for each language (coefficients averaged across 4 reward models $\times$ 4 datasets = 16 runs per language). Unlike the strong positive \textit{between-language} correlation, within-language NLL coefficients are mixed in sign and small in magnitude, indicating that the NLL--score relationship is primarily a \textit{language-level} phenomenon.}
\label{tab:within_language}
\end{table}

==> table/accepted_rejected.tex <==

% \begin{table*}[ht]
% \centering
% \caption{Per-language means (var) by model and setting}
% \label{tab:all_models_stats}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{l r r r r r r r r}
% \toprule
% Language & \multicolumn{2}{c}{Aya} & \multicolumn{2}{c}{Qwen} & \multicolumn{2}{c}{Prometheus 14B} & \multicolumn{2}{c}{Llama 70B} \\ 
%  & accepted & rejected & accepted & rejected & accepted & rejected & accepted & rejected \\ 
% \midrule
% ar & 4.402 (1.524) & 3.781 (2.494) & 4.225 (0.723) & 3.086 (1.834) & 3.346 (2.066) & 2.435 (2.093) & 4.634 (0.667) & 3.450 (2.586) \\ 
% cs & 4.540 (1.082) & 3.853 (2.408) & 4.206 (0.953) & 2.977 (2.016) & 3.627 (2.074) & 2.457 (2.399) & 4.491 (0.787) & 3.297 (2.527) \\ 
% de & 4.645 (0.702) & 3.843 (2.269) & 4.136 (0.910) & 2.932 (1.881) & 3.740 (1.792) & 2.595 (2.397) & 4.479 (0.936) & 3.148 (2.649) \\ 
% el & 4.583 (0.742) & 3.865 (2.135) & 4.239 (0.966) & 3.019 (2.084) & 4.160 (1.680) & 2.838 (2.755) & 4.660 (0.709) & 3.512 (2.689) \\ 
% es & 4.484 (0.894) & 3.709 (2.221) & 4.196 (0.786) & 2.962 (1.828) & 3.718 (1.847) & 2.515 (2.244) & 4.616 (0.740) & 3.312 (2.673) \\ 
% fa & 4.617 (0.571) & 3.921 (1.947) & 4.193 (0.831) & 3.117 (1.821) & 3.911 (1.545) & 2.812 (2.269) & 4.582 (0.802) & 3.477 (2.536) \\ 
% fr & 4.559 (0.696) & 3.731 (2.225) & 4.145 (0.837) & 2.913 (1.815) & 3.715 (1.847) & 2.547 (2.345) & 4.616 (0.712) & 3.254 (2.703) \\ 
% he & 4.114 (2.462) & 3.663 (3.054) & 4.032 (0.989) & 3.067 (1.744) & 3.366 (2.086) & 2.600 (1.948) & 4.693 (0.668) & 3.713 (2.573) \\ 
% hi & 4.772 (0.496) & 4.149 (1.963) & 4.480 (0.637) & 3.365 (2.006) & 3.865 (2.476) & 2.970 (3.155) & 4.671 (0.590) & 3.653 (2.424) \\ 
% id & 4.583 (0.770) & 3.850 (2.188) & 4.104 (0.756) & 2.967 (1.688) & 3.483 (2.013) & 2.502 (2.100) & 4.577 (0.734) & 3.367 (2.533) \\ 
% it & 4.546 (0.814) & 3.725 (2.276) & 4.172 (0.843) & 2.918 (1.831) & 3.671 (1.977) & 2.494 (2.288) & 4.571 (0.766) & 3.228 (2.635) \\ 
% ja & 4.634 (0.629) & 3.876 (2.145) & 4.315 (0.712) & 3.224 (1.748) & 3.596 (1.881) & 2.724 (2.302) & 4.664 (0.780) & 3.466 (2.758) \\ 
% ko & 4.520 (0.794) & 3.869 (1.954) & 4.226 (0.712) & 3.195 (1.763) & 3.716 (1.613) & 2.669 (2.162) & 4.586 (1.030) & 3.571 (2.772) \\ 
% nl & 4.595 (0.616) & 3.818 (2.135) & 4.087 (0.874) & 2.917 (1.826) & 4.049 (1.826) & 2.738 (2.807) & 4.564 (0.853) & 3.217 (2.750) \\ 
% pl & 4.273 (2.079) & 3.629 (3.027) & 4.192 (0.906) & 2.960 (1.920) & 3.896 (2.023) & 2.595 (2.672) & 4.548 (0.766) & 3.245 (2.562) \\ 
% pt & 4.545 (0.804) & 3.731 (2.273) & 4.201 (0.801) & 2.960 (1.850) & 3.721 (1.966) & 2.552 (2.323) & 4.606 (0.713) & 3.295 (2.679) \\ 
% ro & 4.358 (1.591) & 3.646 (2.587) & 4.160 (0.887) & 2.969 (1.868) & 3.920 (1.624) & 2.771 (2.335) & 4.585 (0.774) & 3.314 (2.649) \\ 
% ru & 4.661 (0.887) & 3.978 (2.422) & 4.206 (0.810) & 2.996 (1.876) & 3.888 (1.601) & 2.692 (2.376) & 4.468 (0.848) & 3.291 (2.528) \\ 
% tr & 4.432 (1.044) & 3.741 (2.196) & 4.245 (0.776) & 3.164 (1.827) & 3.693 (1.949) & 2.642 (2.538) & 4.577 (0.829) & 3.466 (2.619) \\ 
% uk & 4.505 (1.502) & 3.881 (2.724) & 4.198 (0.822) & 3.032 (1.883) & 3.821 (1.929) & 2.666 (2.481) & 4.524 (0.936) & 3.433 (2.538) \\ 
% vi & 4.607 (0.703) & 3.899 (2.133) & 4.304 (0.762) & 3.088 (1.934) & 3.897 (1.774) & 2.680 (2.350) & 4.546 (0.765) & 3.403 (2.467) \\ 
% zh & 4.547 (0.851) & 3.806 (2.215) & 4.092 (0.916) & 3.005 (1.785) & 3.806 (1.844) & 2.679 (2.388) & 4.504 (1.018) & 3.322 (2.618) \\ 
% \bottomrule
% \end{tabular}%
% }
% \end{table*}



==> table/pairwise_score.tex <==
\begin{table*}[t]
\centering
\small
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccccccccccccccccc}
\toprule
Model & Avg & Var 
& ar & cs & de & el & es & fa & fr & he & hi & id & it & jp & kr & nl & pl & pt & ro & ru & tr & uk & vi & zh \\
\midrule
LLaMA 3.1 70B 
& 75.5 & 1.4 
& 75.8 & 74.9 & 75.5 & 74.7 & 76.7 & 74.8 & 77.6 & 74.7 & 73.7 & 76.8 & 76.8 & 74.7 & 73.2 & 75.9 & 75.8 & 76.4 & 75.8 & 75.9 & 73.4 & 75.1 & 76.8 & 76.1 \\
Aya Expanse 32B 
& 71.9 & 3.4 
& 70.1 & 73.6 & 71.8 & 69.6 & 72.7 & 68.1 & 72.8 & 70.5 & 70.4 & 73.6 & 73.7 & 71.5 & 67.9 & 72.6 & 73.5 & 73.0 & 73.5 & 73.5 & 70.4 & 73.9 & 72.5 & 72.6 \\
\bottomrule
\end{tabular}
}
\caption{Per-language average scores for LLaMA 3.1 70B and Aya Expanse 32B.}
\label{tab:llama_aya_language_scores}
\end{table*}

==> within_language_effect/table_between_within.tex <==
\begin{table}[h]
\centering

\small
\begin{tabular}{ll rrr}
\toprule
\textbf{Model} & \textbf{Split} & $\beta_B$ & $\beta_W$ & $\beta_{\mathrm{IFE}}$ \\
\midrule
BTRM-Qwen2-7B & Chat & 0.225* & 0.202*** & 0.457*** \\
 & Chat-Hard & 0.310*** & 0.813*** & 0.635*** \\
 & Reasoning & -0.015 & 0.884*** & -0.083** \\
 & Safety & 0.607*** & 0.246*** & 1.214*** \\
\midrule
Skywork-Gemma-27B & Chat & 0.065 & -0.079 & 0.145 \\
 & Chat-Hard & 0.609** & -0.839*** & 2.588*** \\
 & Reasoning & -0.409*** & 1.969*** & -1.435*** \\
 & Safety & 0.778*** & 0.676*** & 1.845*** \\
\midrule
Skywork-LLaMA-8B & Chat & 1.086** & -0.820*** & 3.994*** \\
 & Chat-Hard & 1.677** & -1.495*** & 4.026*** \\
 & Reasoning & 0.465 & 1.588*** & 1.321*** \\
 & Safety & 0.939 & 1.642*** & 1.997*** \\
\midrule
URM-LLaMA-8B & Chat & 0.289* & -1.381*** & 0.788*** \\
 & Chat-Hard & 0.410** & -1.339*** & 0.513*** \\
 & Reasoning & 0.209* & 0.371*** & 0.709*** \\
 & Safety & 0.436*** & 1.145*** & 1.083*** \\
\bottomrule
\end{tabular}
\caption{Between-language vs.\ within-language NLL$\to$Score slopes, and item-fixed-effects estimates. $\beta_B$ is the slope of language-mean score on language-mean NLL; $\beta_W$ is the language-demeaned pooled slope; $\beta_{\mathrm{IFE}}$ is the NLL coefficient after item fixed effects. All slopes are standardized (per 1\,SD of NLL).}
\label{tab:between_within}

\end{table}
